r-softmax: Generalized Softmax with Controllable Sparsity Rate

Nowadays artificial neural network models achieve remarkable results in many disciplines. Functions mapping the representation provided by the model to the probability distribution are the inseparable aspect of deep learning solutions. Although softmax is a commonly accepted probability mapping function in the machine learning community, it cannot return sparse outputs and always spreads the positive probability to all positions. In this paper, we propose r-softmax, a modification of the softmax, outputting sparse probability distribution with controllable sparsity rate. In contrast to the existing sparse probability mapping functions, we provide an intuitive mechanism for controlling the output sparsity level. We show on several multi-label datasets that r-softmax outperforms other sparse alternatives to softmax and is highly competitive with the original softmax. We also apply r-softmax to the self-attention module of a pre-trained transformer language model and demonstrate that it leads to improved performance when fine-tuning the model on different natural language processing tasks.

==> mnistgap.tex <==
\begin{figure*}[ht!]
\vskip 0.1in
\begin{center}
    \includegraphics[width=1.0\textwidth]{images/mse_gap_60_legend}\hfill
    \includegraphics[width=.33\textwidth]{images/mse_60_gap.png}\hfill
    \includegraphics[width=.33\textwidth]{images/mse_40_gap}\hfill
    \includegraphics[width=.33\textwidth]{images/mse_20_gap}\hfill
\caption{The MSE difference on the MNIST validation dataset between the discretized one hot version and its continuous approximation. In contrast to Gumbel-Softmax, in our $\rgumbelfull$, we can avoid the information leakage as we can ensure one hot categorical representation of latent vectors by setting the final sparsity rate~$r$ in~$\ourr$ to~$1 - \frac{1}{|d|}$, where~$d$ is the selected latent size. \label{fig:msegaptest}}
\end{center}
\vskip -0.2in
\end{figure*}


==> plotintro.tex <==
\begin{figure}[tbh!]
\vskip 0.2in
\begin{center}
    \includegraphics[scale=0.4]{introplot.png}
\end{center}
\caption{A comparison between $\ourr$ and softmax in the multi-label classification scenario. The task of both functions is to return the probability distribution over the specified classes, based on the output provided by the neural network model. Since $\ourr$ is able to produce zero probabilities, we can consider them as an indication of a negative class. For softmax, we need to select an appropriate threshold below which a class will be classified as negative. Thus, the representation provided by $\ourr$ is more intuitive and more interpretable. \label{fig:intro}}
\vskip -0.2in
\end{figure}


==> tables/aebinmnist.tex <==
\begin{table*}[t]
\caption{The mean squared error (MSE) of the image reconstruction produced by the Auto-Encoder with binary latent representation provided by Gumbel-Softmax (GS) and $\rgumbelfull$ (r-GS). We report results for different latent sizes $d$ on MNIST and Fashion-MNIST validation set. The presented results indicate that our method meaningfully outperforms the Gumbel-Softmax approach in the scenario when we require a binary representation with a fixed percentage of non-zero bits. \label{tab:binaemnistresults}}
\vskip 0.15in
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{llllllll}
\toprule
 & & \multicolumn{3}{c}{\textbf{MNIST}} & \multicolumn{3}{c}{\textbf{Fashion-MNIST}} \\
\midrule
Latent Size & \makecell[l]{Experiment\\Setup} & \makecell[l]{MSE (\% Hot)\\All Hot} & \makecell[l]{MSE\\5\% Hot} & \makecell[l]{MSE\\10\% Hot} & \makecell[l]{MSE (\% Hot)\\All Hot} & \makecell[l]{MSE\\5\% Hot} & \makecell[l]{MSE\\10\% Hot}\\
\midrule
% LS = 60 \\
% \midrule
\multirow{5}{*}{\begin{tabular}[x]{@{}l@{}}$d=60$ \end{tabular}} 
& GS, $\tau$=[1, 0.1] & 0.216 (2.7\%) & 0.233 & 0.254 & 0.191 (2.1\%) & 0.214 & 0.439 \\
& GS, $\tau$=[1, 0.3] & 0.211 (7.9\%) & 0.241 & 0.274 & 0.155 (6.4\%) & 0.183 & 0.228 \\
& GS, $\tau$=[1, 0.5] & 0.192 (55.3\%) & 0.239 & 0.220 & 0.159 (9.7\%) & 0.191 & 0.295 \\
& r-GS, r=[1, 0.95] & 0.203 (5\%) & 0.203 & - & 0.172 (5\%) & 0.172 & -\\
& r-GS, r=[1, 0.9] & 0.199 (10\%) & - & 0.199 & 0.176 (10\%) & - & 0.176 \\
\midrule
% LS = 40 \\
% \midrule
\multirow{6}{*}{\begin{tabular}[x]{@{}l@{}}$d=40$ \end{tabular}} 
& GS, $\tau$=[1, 0.1] & 0.228 (3.5\%) & 0.235 & 0.244 & 0.224 (3.1\%) & 0.237 & 0.261 \\
& GS, $\tau$=[1, 0.3] & 0.209 (14.3\%) & 0.228 & 0.230 & 0.176 (5.9\%) & 0.209 & 0.240\\
& GS, $\tau$=[1, 0.5] & 0.211 (74.3\%) & 0.275 & 0.243 & 0.173 (37.1\%) & 0.292 & 0.227\\
& r-GS, r=[1, 0.95] & 0.214 (5\%) & 0.214 & - & 0.203 (5\%) & 0.203 & - \\
& r-GS, r=[1, 0.9] & 0.211 (10\%) & - & 0.211 & 0.194 (10\%) & - & 0.194  \\
\midrule
% LS = 20 \\
% \midrule
\multirow{6}{*}{\begin{tabular}[x]{@{}l@{}}$d=20$ \end{tabular}} 
& GS, $\tau$=[1, 0.1] & 0.218 (7.1\%) & 0.230 & 0.230 & 0.203 (5.1\%) & 0.206 & 0.220 \\
& GS, $\tau$=[1, 0.3] & 0.214 (22.6\%) & 0.264 & 0.245 & 0.162 (14.2\%) & 0.268 & 0.206 \\
& GS, $\tau$=[1, 0.5] & 0.210 (72.1\%) & 0.280 & 0.260 & 0.182 (26.0\%) & 0.344 & 0.302\\
& r-GS, r=[1, 0.95] & 0.230 (5\%) & 0.230 & - & 0.279 (5\%) & 0.279 & -\\
& r-GS, r=[1, 0.9] & 0.209 (10\%) & - & 0.209 & 0.211 (10\%) & - & 0.211 \\
\bottomrule
\end{tabular}
% \end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

==> tables/aemnisttable.tex <==
\begin{table}[h!]
\caption{The mean squared error (MSE) of the image reconstruction produced by the Auto-Encoder with a categorical latent representation. We compare the one hot discrete representation (One Hot) with it's approximation (Soft) provided by our $\rgumbelfull$ (r-GS) and Gumbel-Softmax (GS). We present results for different latent sizes $d$ for MNIST and Fashion-MNIST validation set.\label{tab:aemnistresults}}
\vskip 0.15in
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{llllll}
\toprule
&  & \multicolumn{2}{c}{\textbf{MNIST}} & \multicolumn{2}{c}{\textbf{Fashion-MNIST}} \\
\midrule \makecell[l]{Latent\\size ($d$)} &
\makecell[l]{Experiment\\Setup} & \makecell[l]{MSE\\One\\Hot} & \makecell[l]{MSE\\Soft} & \makecell[l]{MSE\\One\\Hot} & \makecell[l]{MSE\\Soft} \\
\midrule
% $d = 60$ \\ 
% \midrule

\multirow{6}{*}{\begin{tabular}[x]{@{}l@{}}60 \end{tabular}} 
& GS, t=[1, 0.1] & 0.162 & 0.157 & 0.116 & 0.113 \\
& GS, t=[1, 0.3] & 0.180 & 0.141 & 0.133 & 0.102 \\
& GS, t=[1, 0.5] & 0.193 & 0.121 & 0.151 & 0.088 \\
& r-GS r=[1, $\frac{1}{d}$] & 0.173 & 0.173 & 0.134 & 0.134 \\
& r-GS, r=[1, 0.05] & 0.193 & 0.137 & 0.148 & 0.093 \\
& r-GS, r=[1, 0.1] & 0.211 & 0.117 & 0.167 & 0.080 \\
\midrule
% $d = 40$ \\ 
% \midrule
\multirow{6}{*}{\begin{tabular}[x]{@{}l@{}}40 \end{tabular}} 
& GS, t=[1, 0.1] & 0.171 & 0.166 & 0.121 & 0.124 \\
& GS, t=[1, 0.3] & 0.188 & 0.149 & 0.144 & 0.110 \\
& GS, t=[1, 0.5] & 0.206 & 0.128 & 0.161 & 0.093\\
& r-GS, r=[1.0,$\frac{1}{d}$] & 0.179 & 0.179 & 0.136 & 0.136\\
& r-GS, r=[1, 0.05] & 0.187 & 0.156 & 0.137 & 0.110\\
& r-GS, r=[1, 0.1] & 0.207 & 0.133 & 0.172 & 0.090 \\
\midrule
% $d = 20$ \\ 
% \midrule
\multirow{6}{*}{\begin{tabular}[x]{@{}l@{}}20 \end{tabular}} 
& GS, t=[1, 0.1] & 0.188 & 0.182 & 0.141 & 0.135 \\
& GS, t=[1, 0.3] & 0.207 & 0.158 & 0.164 & 0.118 \\
& GS, t=[1, 0.5] & 0.218 & 0.136 & 0.184 & 0.102\\
& r-GS, r=[1.0,$\frac{1}{d}$] & 0.195 & 0.195 & 0.152 & 0.152 \\
& r-GS, r=[1, 0.05] & 0.195 & 0.195 & 0.152 & 0.152 \\
& r-GS, r=[1, 0.1] & 0.201 & 0.165 & 0.161 & 0.119\\
\bottomrule
\end{tabular}
% \end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

==> tables/vqvae.tex <==
\begin{table}[t]
\caption{The mean squared error (MSE) of the image reconstruction produced by the VQ-VAE modification on Cifar10.  We compare the  discrete (One Hot) and continuous (Soft) representation provided by Gumbel-Softmax (GS) and $\rgumbelfull$ (r-GS). We can observe that if we allow the model to select more than one embedding to represent the elements in the hidden representation (Soft), our model achieves better results (even if it can select only 5\% of the embeddings). \label{tab:vqvae}}
\vskip 0.15in
\begin{center}
\begin{small}
% \begin{sc}
\begin{tabular}{lll}
\toprule
Experiment Setup & \makecell[l]{MSE\\One Hot} & \makecell[l]{MSE\\Soft}\\
\midrule
% GS, t=[1, 0.1], $\lambda=0.001$ & 2.70 $\cdot10^{-4}$ & 2.64 $\cdot10^{-4}$ \\
% GS, t=[1, 0.1], $\lambda=0.0001$ & 2.74 $\cdot10^{-4}$ & 2.66 $\cdot10^{-4}$ \\
GS, $\tau$=[1, 0.1] & 2.70 $\cdot10^{-4}$ & 2.64 $\cdot10^{-4}$ \\
% GS, t=[1, 0.3], $\lambda=0.001$ & 2.82 $\cdot10^{-4}$ & 2.41 $\cdot10^{-4}$ \\
% GS, t=[1, 0.3], $\lambda=0.0001$ & 2.85 $\cdot10^{-4}$ & 2.49 $\cdot10^{-4}$ \\
GS, $\tau$=[1, 0.3] & 2.82 $\cdot10^{-4}$ & 2.41 $\cdot10^{-4}$ \\
% GS, t=[1, 0.5], $\lambda=0.001$ & 3.07 $\cdot10^{-4}$ & 1.98 $\cdot10^{-4}$\\
% GS, t=[1, 0.5], $\lambda=0.0001$ & 2.91 $\cdot10^{-4}$ & 2.13 $\cdot10^{-4}$\\
GS, $\tau$=[1, 0.5] & 3.07 $\cdot10^{-4}$ & 1.98 $\cdot10^{-4}$ \\
% R-GS, r=[1, 0.1], $\lambda=0.001$ & 4.40 & 1.29 \\
% R-GS, r=[1, 0.1], $\lambda=0.0001$ & 3.97 & 1.54 \\
r-GS, r=[1, 0.9] & 4.40 $\cdot10^{-4}$ & 1.29 $\cdot10^{-4}$ \\ 
% R-GS, r=[1, 0.05], $\lambda=0.001$ & 4.32 & 1.24 \\
% R-GS, r=[1, 0.05], $\lambda=0.0001$ & 4.01 & 1.56 \\
r-GS, r=[1, 0.95] & 4.32 $\cdot10^{-4}$ & 1.24 $\cdot10^{-4}$ \\
% R-GS, r=[1, $\frac{1}{d}$], $\lambda=0.001$ & 3.81 & 1.64 \\
% R-GS, r=[1, $\frac{1}{d}$], $\lambda=0.0001$ & 3.67 & 2.09 \\
r-GS, r=[1, $1 - \frac{1}{d}$] & 3.81 $\cdot10^{-4}$ & 1.64 $\cdot10^{-4}$ \\
\bottomrule
\end{tabular}
% \end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}
